COFS: Controllable Furniture layout Synthesis

Scalable generation of furniture layouts is essential for many applications in virtual reality, augmented reality, game development and synthetic data generation. Many existing methods tackle this problem as a sequence generation problem which imposes a specific ordering on the elements of the layout making such methods impractical for interactive editing or scene completion. Additionally, most methods focus on generating layouts unconditionally and offer minimal control over the generated layouts. We propose COFS, an architecture based on standard transformer architecture blocks from language modeling. The proposed model is invariant to object order by design, removing the unnatural requirement of specifying an object generation order. Furthermore, the model allows for user interaction at multiple levels enabling fine grained control over the generation process. Our model consistently outperforms other methods which we verify by performing quantitative evaluations. Our method is also faster to train and sample from, compared to existing methods.

==> COFS_ Controllable Furniture Layout Synthesis/sections/conclusion.tex <==
\section{Conclusions}
We proposed a new framework to produce layouts with auto-regressive transformers with arbitrary conditioning information. While previous work was only able to condition on a set of complete objects, we extend this functionality and also allow for conditioning on individual attributes of objects. Our framework thereby enables several new modeling applications that cannot be achieved by any published framework.


\paragraph{Societal Impact.} We do not expect any negative social impact that is directly linked to our work. We do acknowledge possible concerns about the energy consumption of training auto-regressive transformers.

\paragraph{Limitations and Future Work.}
Our work inherits some limitations of auto-regressive models (or even generative models in general) in that we require long training times and that setting up the code is laborious, time-consuming and error-prone. In addition, it requires significant expert knowledge in training transformers. We will therefore release the code upon acceptance. Another limitation of the work is that all objects need to have the same number of attributes. An open challenge for future work is to extend our approach to layouts where each object is described by a token sequence of variable length.
Further, we would like to work on scaling auto-regressive models to much larger sequences, e.g., by using hierarchical auto-regressive models. In future, we would also like to explore parallel sampling strategies to sidestep the slow autoregressive generation process.

%\subsection{Limitations}
%While the 

\begin{table}[t]
\centering
\small
\caption{\textbf{Comparison on Synthesis Time}: We compare the time required to synthesize a single scene for different categories. Our model outperforms all other models on this metric, and is competitive on FID in comparison to ATISS. Our model achieves this while being parameter efficient. We only have about half the parameters of the next closest competitor. About 10m of these parameters come from the ResNet-18 encoder.}
\setlength\tabcolsep{2pt}
\begin{tabular}{@{}lcccccccc|c@{}}
\toprule
\multicolumn{1}{l}{} & \multicolumn{4}{c}{Synthesis Time ($\downarrow$)}                                 & \multicolumn{4}{c|}{FID ($\downarrow$)}                                              & \multirow{2}{*}{\begin{tabular}{c}
                                             Params  \\
                                             ($\downarrow$)
                                        \end{tabular}}   \\

\cmidrule(l){2-5} \cmidrule(l){6-9} 
                  & \bed             &  \liv         & \din           & \lib                           & \bed             & \liv          & \din              &  \lib                           & \\ \midrule
{FastSynth}       & 13193.77         &  30578.54     & 26596.08       & \multicolumn{1}{c|}{10813.87}  &  88.1             & 66.6           & 58.9             & \multicolumn{1}{c|}{ 86.6}         &  38.1  \\
{SceneFormer}     & 849.37           &  731.84       &  901.17        &  \multicolumn{1}{c|}{369.74}   &  90.6             & 68.1           & 60.1           & \multicolumn{1}{c|}{ 89.1}            & 129.29 \\
{ATISS}           & 102.38           &  201.59       &  201.84        & \multicolumn{1}{c|}{88.24}     &  \textbf{73.0 }  & 43.32         & 47.66           & \multicolumn{1}{c|}{\textbf{ 75.34}}       & 36.05      \\%
{Ours}            &  \textbf{33.69}  &\textbf{77.37} &\textbf{76.75}  & \multicolumn{1}{c|}{ \textbf{29.32}}  &  73.2            &\textbf{35.9} &\textbf{43.12}  & \multicolumn{1}{c|}{75.72}           & \textbf{19.44} \\
\bottomrule
\end{tabular}
\vspace{-0.1cm}
\end{table}


==> COFS_ Controllable Furniture Layout Synthesis/sections/introduction.tex <==
\section{Introduction}
Automatic generation of realistic assets enables content creation at a scale that is not possible with traditional manual workflows. It is driven by the growing demand for virtual assets in both the creative industries, virtual worlds, and increasingly data-hungry deep model training. 3D scene and layout generation plays a central role in automatic asset generation, as much of the demand is for the types of real-world scenes we see and interact with every day, such as building interiors.

Deep generative models for assets like images, videos, 3D shapes, and 3D scenes have come a long way to meet this demand. 
%Generative models have come a long way to generate high quality images, videos, objects, and 3D scenes.
In the context of 3D scene and layout modeling, in particular auto-regressive models based on transformers enjoy great success. Inspired by language modeling, these architectures treat layouts as sequences of tokens and are particularly well suited for modeling spatial relationships between elements of a layout. For example, Para et al.~\cite{para} generate two-dimensional interior layouts with two transformers, one for furniture objects and one for spatial constraints between these objects, while SceneFormer~\cite{wang2021sceneformer} extends interior layout generation to 3D.

A main limitation of these approaches is that they do not support scene completion from arbitrary partial scenes, due to their need for a consistent sequence ordering. In bedroom layouts, for example, the bed always needs to be generated before the nightstands, which precludes completing scenes that already have nightstands, but are missing a bed. ATISS~\cite{Paschalidou2021NEURIPS}, which is the most current layout generation approach, tackles this problem by randomly permuting the token sequence during training, enabling scene completion from arbitrary subsets of objects.

%. In these methods, the sequence representation of a scene needs to have a consistent ordering (in bedroom layouts, for example, the bed always needs to be generated before the nightstands), therefore a scene that already has nightstands in it cannot 

%sequences need to 

%ATISS~\cite{ATISS} is the most current approach. 

%The main idea is to enable 

%The two main ideas are to shorten the token sequence by using one token per objects instead of 

%(Many of these architecture ideas are inspired by language modedling).
%One idea is to model objects and constraints with separate transformers (Wamiq ICCV 2021)

%MaskGit

%Scene Former

%ATIS is the most current model. The two main ideas are to encode each object as one token, opposed to enconding each attribute as separate token. Therefore the model uses fewer tokens to describe a scene. The second main idea is to enable sampling objects in arbitrary order and conditioning on objects given in arbitrary order (conditioning on arbitrary subset of objects).

While ATISS works well, we aim to improve on these results to enable more fine grained conditioning. We want to keep the advantage of conditioning on arbitrary subsets of objects, but we also want to extend to conditioning on arbitrary subsets of attributes. For example, a user might be interested to ask for a room with a table and two chairs, without specifying exactly where these objects should be located. Another example is to perform object queries for given geometry attributes. The user could specify the location of an object and query the most likely class, orientation, and size of an object at the given location. Our model thereby extends the baseline ATISS with new functionality while retaining all its existing properties and performance.

The main technical difficulty in achieving a more fine-grained conditioning is due to the autoregressive nature of the generative model. Tokens in the sequence that define a scene are generated iteratively, and each step only has information about the previously generated tokens. Thus, the condition can only be given at the start of the sequence, otherwise some generation steps will miss some of the conditioning information.
%
The main idea of our work is to allow for fine-grained conditioning using two mechanisms: (i)~Like ATISS, we train our generator to be approximately permutation-invariant and provide the condition as partial sequence that needs to be completed by the generative model.
Unlike previous work, the condition is not restricted to the start of the sequence, which means that some tokens do not have full information about the condition through the autoregressive generator alone. (ii)~To give our autoregressive model knowledge of the entire conditioning information in each step, we additionally use a transformer encoder that provides cross-attention over the complete conditioning information in each step. These two mechanisms allow us to accurately condition on arbitrary subsets of the token sequence, for example, only on tokens corresponding to specific object attributes.

%both through a transformer encoder and by manually fixing a subset of the object sequence.

%- add a transformer encoder that encodes the partial scene and allows the transformer to plan ahead for , while also manually 

In our experiments, we demonstrate four applications: (i) outlier detection, (ii) unconditional generation, (iii) traditional scene completion from a partial set of objects, and (iv) fine-grained conditioning on a subset of object attributes. We compare to three current state-of-the-art layout generation methods~\cite{fastsynth:ritchie,wang2021sceneformer,Paschalidou2021NEURIPS} and show performance that is on par or superior, while also enabling fine-grained conditioning, which, to the best of our knowledge, is currently not supported by any existing layout generation method.

%show that we can use this method to successfully complete scenes given a list of partial object attributes. ...

%(Insert Figure to compare ATISS and New Model)






% To summarize, our contributions are:
% \begin{enumerate}
%     \item Proposing a Masked Language Model for heterogeneous tokens instead of homogeneous tokens.
%     \item A strategy for augmenting the token sequence to let the transformer distinguish between different objects and different token types.
%     \item Using MLM scoring to identify outliers in a set which enables failure correction.
%     \item Breaking the Autoregressive nature of ATISS and enabling arbitrary conditioning order.
% \end{enumerate}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.8\linewidth, height=1in]{figures/arch.png}
%     \caption{Schematic representation of our proposed method.}
%     \label{fig:architecture}
    
% \end{figure*}



% \newlength{\mywidth}
% \newsavebox{\mybox}
% \begin{figure*}
%     \centering
%     \savebox{\mybox}{\includegraphics[width=\linewidth]{figures/retrieval_clearcoat_transparent.png}}
%     % \settowidth{\mywidth}{\usebox{\mybox}}
%     \includegraphics[width=0.29\linewidth]{sections/retrieval_glossy_bsdf_walls_shadow_attempt2.png}
%     \includegraphics[width=0.29\linewidth]{sections/retrieval_glossy_bsdf_walls_shadow_attempt2.png}
%     \caption{Examples of our generated floorplans.}
%     \label{fig:my_label}

% \end{figure*}

% \begin{figure}
%     \centering
%     \fcolorbox{black}{gray!30}{\includegraphics{figures/blank.pdf}}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

==> COFS_ Controllable Furniture Layout Synthesis/sections/method.tex <==
\section{Method}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth, height=1.67in]{figures/arch2.pdf}
 \caption{COFS Overview. (\textbf{Left}): The model is a BART-like encoder-decoder model, with a bidirectional encoder and an autoregressive decoder. Note the attention matrices shown in grey. At training time, a permutation $\pi$ permutes the objects in a scene. The encoder receives additional information in the form of \textit{Relative Position Tokens} $\mathcal{R}^i$, and the \textit{Object Index Tokens} $\mathcal{O}^i$.  A random proportion of tokens is replaced with a \mask token. The decoder is trained with \textit{Absolute Position Tokens} $\mathcal{P}^i$ and performs two tasks - 1. copy-paste: the attributes should be sampled at the proper location 2: mask-prediction: the decoder predicts the actual value of the token corresponding to a \mask token in the encoder sequence. (\textbf{Right}): During inference, to measure likelihood, we create a copy of the sequence with each token masked out. The decoder outputs a probability distribution over the possible values of the masked tokens.}
    \label{fig:architecture}
\end{figure*}

%In this example, we use 2 object attributes and $n$ objects.

Our goal is to design a generative model of object layouts that allows for fine-grained conditioning on individual object attributes. Fine-grained conditioning enables more flexible partial scene specification, for example specifying only the number and types of objects in a scene, but not their positions, or exploring suggestions for plausible objects at given positions in the layout.

% the following three paragraphs are similar to the intro, they can be moved to the intro to replace the current paragraphs in the intro, or be commented out if we need more space or think this is too much repetition

\paragraph{Generative model.} We use a transformer-based generative model, as these types of generative models have shown great performance in the current state of the art. Originally, proposed as a generative model for language, transformer-based generative models represents layouts as a sequence of tokens $S=(s_1, \dots, s_n)$ that are generated auto-regressively; one token is generated at a time, based on all previously generated tokens:
\begin{equation}
    p(s_i | S_{<i}) = f_\theta(S_{<i}),
\end{equation}
where $p(s_i | S_{<i})$ is the probability distribution over the value of token $s_i$, computed by the generative model $f_\theta$ given the previously generated tokens $S_{<i} = (s_1, \dots, s_{i-1})$.
We sample from $p(s_i | S_{<i})$ to obtain the token $s_i$.
Each token represents one attribute of an object, and groups of adjacent tokens correspond to objects. More details on the layout representation are described in Section~\ref{sec:layout_rep}.

\paragraph{Conditioning.} To condition a transformer-based generative model on a partial sequence $C$, we can replace tokens of $S$ with the corresponding tokens of $C$, giving us the sequence $S^C$. This is done after each generation step, so that the probability for the token in each step is conditioned on $S^C_{<i}$ instead of $S_{<i}$:
\begin{eqnarray}
    p(s_i | S^C_{<i}) = f_\theta(S^C_{<i}).
\end{eqnarray}
%where $\mathbf{1}$ is the indicator function, and $c_i$ is element $i$ of C.
Each generated token $s_i$ in $S^C$ (i.e. tokens that are not replaced by tokens in $C$) needs to have knowledge of the full condition during its generation step, otherwise the generated value may be incompatible with some part of the condition. Therefore, since each generated token $s_i$ only has information about the partial sequence $S^C_{<i}$, the condition can only be given as start of the sequence:
\begin{equation}
S^C =
\begin{cases}
c_i \text{ if } i \le |C| \\
s_i \text{ otherwise}.
\end{cases}
\end{equation}
%, , so that all generated tokens $S_{>|C|}$ have full knowledge of the condition.

\paragraph{Conditioning without permutation invariance.} Typically both the objects and the attributes of the objects in the sequence are consistently ordered according to some strategy, for example based on a raster order of the object positions~\cite{para}, or on the object size~\cite{planit:wang}. Therefore, a generative model $f^{\text{ordered}}_\theta$ that is only trained to generate sequences in that order cannot handle different orderings, so that in general:
\begin{equation}
    f^{\text{ordered}}_\theta(S^C_{<i}) \neq f^{\text{ordered}}_\theta(\pi_o(S^C_{<i})),
\end{equation}
where $\pi_o$ is a random permutations of the objects in sequence $S_{<i}$. The consistent ordering improves the performance of the generative model, but also presents a challenge for conditioning:
%since each generated token $s_i$ only has information about the previously generated tokens $S_{<i}$, a condition $C \subset S$, such as a partial set of objects, can only be given as start of the sequence $C = S_{<j}$, so that all subsequently generated tokens $S_{\ge j}$ have full access to the condition:
% \begin{equation}
%     p(s_i) = f_\theta(s_i | S_{<i}),
%     f^{\text{ordered}}_\theta(s_i | S_{<i}) \neq f^{\text{ordered}}_\theta(s_i | \pi_o(S_{<i})),
% \end{equation}
%Thus,
the consistent sequence ordering limits the information that can appear in the condition. In a bedroom layout, for example, if beds are always generated before nightstands in the consistent ordering, the layout can never be conditioned on nightstands only, as this would preclude the following tokens from containing a bed.

\paragraph{Permutation invariance for more general conditioning.} Recent work~\cite{Paschalidou2021NEURIPS} tackles this issue by forgoing the consistent object ordering, and instead training the generator to be approximately invariant to permutations $\pi_o$ of objects in the sequence:
\begin{equation}
    f_\theta(S^C_{<i}) \approx f_\theta(\pi_o(S^C_{<i})),
\end{equation}
This makes generation more difficult, but allows conditioning on arbitrary subset of objects, as now arbitrary objects can appear at the start of the sequence. However, since only objects are permuted and not their attributes, it does not allow conditioning on subsets of object attributes. Permuting object attributes to appear at arbitrary positions in the sequence is not a good solution to obtain a more fine-grained conditioning, as this would make it very hard for the generator to determine which attribute corresponds to which object.

\paragraph{Fine-grained conditioning.} We propose to extend previous work to allow for fine-grained conditioning by using two different conditioning mechanisms, in addition to the approximate object permutation invariance: First, similar to previous work, we provide the condition as partial sequence $C$. To allow conditioning on only a subset of the object attributes, we introduce special mask tokens $\mathcal{M}$ in $C$ that denote tokens that are not constrained by $C$. The constrained sequence $S^C$, is then defined as:
%by replacing mask tokens in $C$ with generated tokens:
\begin{equation}
S^C =
\begin{cases}
c_i \text{ if } i \le |C| \text{ and } c_i \neq \mathcal{M} \\
s_i \text{ otherwise}.
\end{cases}
\end{equation}
% However, 
% allow replacing arbitrary tokens in $C$, for example individual object attributes, with special mask tokens $\mu$. During sequence generation, these mask tokens are replaced by generated tokens:
% \begin{eqnarray}
%     p(s_i | S_{<i}, C) = \begin{cases}
%     \mathbf{1}_{\{c_i\}}(s_i) \text{ if } i \le |C| \text{ and } c_i \neq \mu\\
%     f_\theta(S_{<i} ) \text{ otherwise.}
%     \end{cases}
% \end{eqnarray}
Second, to provide information about the full condition to each generated token, including those that replace mask tokens, we modify $f_\theta$ to use a transformer encoder $g_\phi$ that encodes the condition $C$ into a set of feature vectors that each generated token has access to:
\begin{equation}
p(s_i | S^C_{<i}, C) = f_\theta(S^C_{<i}, C^g) \text{ where } C^g = \{g_\phi(c_1, C), \dots, g_\phi(c_{|C|}, C)\},
\label{eq:final_objective}
\end{equation}
where $C^g$ is the output of the encoder, a set of encoded condition tokens. We use a standard transformer encoder-decoder setup~\cite{vaswani} for $f_\theta$ and $g_\phi$, implementation details are provided in Section~\ref{sec:implementation}, and the complete architecture is described in detail in the appendix.


%The objective is to have a generative model of layouts. We desire the following properties - permutation invariance, fast sampling, fast likelihood evaluation. A normal language model will have a position encoding to account for the left-to-right (or the reverse) nature of language. If we remove this - we get a permutation invariant network as attention blocks themselves are permutation invariant. But this treats all tokens the same, which is not what we expect the network to model. There is a difference between the different parameters of a a layout and the network should have that built-in by design. Furthermore, the network should ensure that different token groups have different affinities - change in params of one object should affect the other params of that object more unless there is a global effect (which is modeled by the full attention matrix). As an example - making an object smaller should not change the positions of other objects, while making it larger might need movement of others to avoid intersections. To address each of these problems we introduce additional tokens to inject this bias into our representation and create an \emph{object-centric representation} instead of a \emph{token-centric representation} that is common in standard Language Modelling (LM). 

\subsection{Layout Representation}
\label{sec:layout_rep}
%\subsection{Problem Formulation}
\paragraph{Parameters.}

%WARNING
%\begin{wrapfigure}{l}{0.5\textwidth}
%   \centering
%     \includegraphics[width=0.5\textwidth]{figures/val_losses_v2.pdf}
%     \caption{TODO: INSERT CAPTION}
% \end{wrapfigure}

We focus on 3D layouts in our experiments. A 3D layout $\cL = (\cI, \cB)$ is composed of two elements - a top-down representation of the layout boundary $\cI$, such as the walls of a room, and a set of $k$ three-dimensional oriented bounding-boxes $\cB = \set{B}{i}{1}{k}$ of the objects in the layout. The boundary is given as a binary raster image and each bounding box is represented by four attributes: $B_i = (\tau_i, t_i, e_i, r_i)$, representing the object class, center position, size, and orientation, respectively. The orientation is a rotation about the up-axis, giving a total of 8 scalar values per bounding box. This setup is the same as ATISS.

\paragraph{Layout sequence.}
A layout sequence $S$ is defined by randomizing the order of the bounding boxes, concatenating their parameters, and adding special start and stop tokens $\texttt{SOS}$ and $\texttt{EOS}$ to mark the start and the end of a sequence: $S = [\texttt{SOS}; B_{\pi_1}; \dots; B_{\pi_k}; \texttt{EOS}]$, where $\pi$ is a permutation of the object indices $1, \dots, k$ and $[;]$ denotes concatenation. Note that the objects are permuted in $S$, while the parameters of each object have a consistent order.
The condition $C$ for a layout can be any sub-sequence $S_{<i}$ of $S$, where some tokens may be replaced by mask tokens $\mathcal{M}$, leaving them unconstrained. During training and sampling, these tokens are replaced by generated token.
%, and the model generates a probability distribution over the masked attribute..

\paragraph{Parameter probability distributions.}
The generative model outputs a probability distribution over one scalar component of the bounding box parameters in each step. Similar to previous work~\cite{Paschalidou2021NEURIPS, Salimans2017PixeCNN}, we represent probability distributions over continuous parameters, like the center position, size, and orientation, as mixture of $T$ logistic distributions. Probability distributions over the discrete object class $\tau$ are represented as vectors over logits $l_\tau$ over discrete choices that can be converted to probabilities with the $\text{softmax}$ function.
\begin{equation}
    p(b) = \frac{1}{\sum_i \pi_i} \sum_{i=1}^{T} \alpha_i \text{Logistic}(\mu_i, \sigma_i), \qquad\qquad p(\tau) = \text{softmax}(l_\tau),
    \label{eq:probab}
\end{equation}
where $b$ is a component of $t_i$, $e_i$, or $r_i$, and $\alpha$, $\mu$, $\sigma$, respectively are the mixture weight, mean and variance of the component logistic distributions. Each probability distribution over a continuous scalar component is parameterized by a $3T$-dimensional vector, and probability distributions over the object class are represented as $n_\tau$-dimensional vectors, where $n_\tau$ is the number of object classes.

% , which is output by the generative model $f_\theta$ in each step.
%The center position, size and orientation are in 3D. 

% \paul{TODO: @Wamiq some more bullet points describing the sequence conversion might be useful, like quantization and any other details.}
% The layout boundary is never generated and only provided as condition, details are given in Section~\ref{sec:implementation}.

%location and orientation of a specific class of object in 3D-space. Specifically, $C=\{1, \ldots, n\}$ is the class of the object within the bounding-box, $T \in \nR^3$ is the position vector of the centroid of the bounding-box, $S \in \nR^3$ is vector representing the extent of the bounding-box and $R \in \nR$ is the rotation the bounding-box around the z-axis. We have dropped subscripts for clarity. This is the same parametric representation as ATISS. 

%Conditioned on the floorplan-boundary, there exists a distribution of bounding-boxes within the boundary, obeying the density function $p( \cB | \cI)$. We seek to train a model $f_{\Theta}$ with parameters $\Theta$  that allows us to sample from this distribution:

% \begin{equation}
%     f_{\Theta} \left( \cB | \cI\right) = f\left( \cB | \cI; \Theta\right) = p( \cB | \cI)
% \end{equation}

% Now given a dataset of $N$ scenes, $\cD = \set{\cS}{i}{1}{N}$, we can train our model parameters such that the (log-) likelihood of the observed data is maximized. That is we seek to find the solution $\Theta^*$ that solves the following problem:

% \begin{equation} \label{eq:objective}
%         \Theta^* = \argmax_\Theta \prod_{i=1}^{N}f_{\Theta} \left( \cB_i | \cI_i \right) = \argmin_\Theta \left( \sum_{i=1}^{N} -\log f_{\Theta} \left( \cB_i | \cI_i \right) \right)
% \end{equation}

% Classically [cite niessner, ritchie], in order to the make the likelihood-estimation tractable, the set $\cB_i$ is flattened into a sequence $b = \seq{B}{i}{1}{k}$ under some canonical ordering - raster order as in cite niessner or based on object frequencies as in cite ritchie. This removes ambiguities arising from multiple permutations and makes the task significantly easier. Then, the likelihood can can be factorized in an autoregressive fashion
% \begin{equation}
%     f_{\Theta}(b | \cI) = \prod_{j=1}^{|b|}f_{\Theta}\left( b_j | b_{<j}, \cI \right)
% \end{equation}
% Here, $f_{\Theta}(b_j| b_{<j}, \cI)$ is the probability of the $j$-th object $b_j$ conditioned on  the $j-1$ objects $b_{<j}$. This formulation has certain problems when sampling - if the network has not seen ordering of the partial sequence during training, it will assign a meaningless probability to the current element to be generated. As a concrete example, if the ordering of objects is in the raster order from top-left to bottom-right, and we condition on a sequence that only contains objects from the bottom-right, the model usually assumes the sequence has ended and stops generation. This is the problem of the networks not being permutation invariant.

% despoina create a permutation invariant model called ATISS. ATISS considers an autoregressive model for $f_{\Theta}$ but tries to maximize the likelihood for \emph{all} ordered permutations of the \emph{all} subsets of $\cB_i$, that is 
% \begin{equation}\label{eq:atiss:likelihood}
%     f_{\Theta} \left( \cB | \cI \right) = \prod_{\overline{\cB} \in \pi(\cB)} \prod_{j=1}^{|\overline{\cB}|} f_{\Theta}(\overline{B}_j| \overline{B}_{<j}, \cI)
% \end{equation}

% The function $\pi(\cdot)$ generates a permutation of the input set. This formulation allows for estimating the log-likelihood via a Monte-Carlo approach and as the likelihood is maximized for each \emph{partial} subset $\overline{B}_{<j}$, it allows for partial set completion without any ordering constraints for the partial subset.

% However, the approach still has a major drawback - the sampling process is autoregressive in the order of generation of the attributes. This means that in this model, we cannot condition on an arbitrary subset of attributes. Thus we need to add a term that allows us to condition on an arbitrary subset of suppllied attributes. Inspired by BERT/BART,  we \emph{mask} out a few elements of the set and maximize the likelihood of predicting the masked elements. The other attributes are considered fixed. We replace few chosen attributes at random with a special \mask attribute. A mask $\cM$ is a list of indices of which attributes to replace with \mask. Let the set obtained from $\cB$ after masking be $\cB_{\cM}$. Then the new objective is 

% \begin{equation}\label{eq:our_objective}
%     f_{\Theta} \left( \cB | \cI \right) = \prod_{\overline{\cB} \in \pi(\cB)} \prod_{j \in \cM} f_{\Theta}(\overline{B}_j|\overline{B}_{<j},  \overline{\cB}_{\cM}, \cI)
% \end{equation}

% We find empirically that just maximizing this objective does not lead to good convergence. Thus, instead of just maximizing the likelihood of masked attributes, we maximize the likelihood of all attributes. This gives the modified objective

% \begin{equation}
%     f_{\Theta} \left( \cB | \cI \right) = \prod_{\overline{\cB} \in \pi(\cB)} \prod_{j =1}^{|\overline{\cB}|} f_{\Theta}(\overline{B}_j| \overline{B}_{<j}, \overline{\cB}_{\cM}, \cI)
%     \label{eq:final_objective}
% \end{equation}

% Note that the objective in Eq. \ref{eq:final_objective} leads to two tasks: 1. mask-prediction of the masked tokens and 2. copy-paste of the unmasked tokens.

% TODO: write about sampling $\cM$ from a distribution.

\subsection{Implementation}
\label{sec:implementation}

%Now we describe how the transformer-based generative model $f_\theta$ and the transformer encoder $g_\phi$ are implemented.
%Now we describe how each of the parts in the objective Eq. \ref{eq:final_objective} are implemented.
%We use a BART~\cite{lewis-etal-2020-bart}-like architecture, where the encoder is permutation-invariant, and the generative model predicts the sequence one token at a time. BART is often used for machine translation, and in that setting usually receives the source language in the encoder, and outputs the target language using the generative model. In our setting, we receive the partial layout as condition in the encoder and complete the missing parts using the generative model.

%On a high level, we use a BART-like model for generation. We want the conditioning to be permutation-invariant, hence we remove absolute positional embeddings from the encoder. These are present in the decoder. BART is often used for machine translation, and in that setting usually receives the source language on the encoder, and target language on the decoder. We use BART for generation, and our encoder and decoder receive the same input, with some minor differences that we explain below. With our modifications the encoder represents a set (of conditions and masks), while the decoder samples a sequence. Thus, our task is a \textbf{Masked Set-to-Sequence prediction} task. 

\para{Condition encoder $g_\phi$} To encode the condition $C$ into a set of encoded condition tokens $C^g$, we use a Transformer encoder with full bidirectional attention. As positional encoding, we provide two additional sequences: \emph{object index tokens} $\mathcal{O}^i$ provide for each token the object index in the permuted sequence of objects; and \emph{relative position tokens} $\mathcal{R}^i$ provide for each token the element index inside the attribute tuple of an object. Since the attribute tuples are consistently ordered the index can be used to identify the attribute type of a token. These sequences are used as additional inputs to the encoder. The encoder architecture is based on BART~\cite{lewis-etal-2020-bart}, details are provided in the appendix.

\para{Boundary encoder $g^\mathcal{I}_\psi$} To allow conditioning on the layout boundary $\mathcal{I}$, we prepend a feature vector encoding of the boundary to the input of the condition encoder, as shown in Figure~\ref{fig:architecture}. Similar to ATISS, we use an untrained ResNet-18~\cite{resnet} to encode a top-down view of the layout boundary into an embedding vector.

% , which makes the encoder fully permutation-invariant. However, we found that giving the encoder some prior knowledge about the semantics of tokens is needed to yield good samples. We provide two additional sequences as positional embeddings to the encoder:
% %set representation $C^g$, we use a Transformer Encoder with full bidirectional attention.
% %Without any form of positional encoding, a standard transformer is fully permutation invariant. However, we find that some prior knowledge is needed to yield good samples. We provide two such sources of injecting information: 
% \emph{Object Index Tokens} ($\mathcal{O}^i$), consisting of We assign each object in the permuted set an index and 2. \emph{Relative Position Tokens} ($\mathcal{R}^i$): To each attribute of an object, we assign a canonical position. Note that all these additional tokens are permutation-invariant. The embeddings for one attribute are generated by summing up all the corresponding embeddings. %

\para{Generative model $f_\theta$} The generative model is implemented as a Transformer decoder with a causal attention mask.
%sequence decoder implements autoregressive decoding and is a Transformer Decoder with a causal attention mask.
Each block of the decoder performs cross-attention over the encoded condition tokens $C^g$. As positional encoding, we provide \emph{absolute position tokens} $\mathcal{P}$, which provide for each token the absolute position in the sequence $S$. This sequence is used as additional input to the generative model. The output of the generative model in each step is one of the parametric probability distributions described in Eq.~\ref{eq:probab}. Since the probability distributions for discrete and continuous values have a different numbers of parameters, we use a different final linear layer in the generative model for continuous and discrete parameters. Similar to the encoder, the architecture of the generative model is based on BART~\cite{lewis-etal-2020-bart}.
%activations of the final hidden layer of the Set Encoder.
%We reuse the \textit{unmasked} embeddings generated for encoder side, without embeddings for $\mathcal{R}^i$ and $\mathcal{O}^i$. Instead, we use full \textbf{Absolute Position Tokens} ($\mathcal{P}$) which is standard in Language Modelling. %The sequence is enclosed in \texttt{SOS} and \texttt{EOS} embeddings to denote the start and end of the sequence respectively.
% \para{Boundary encoder $g^\mathcal{I}_\psi$} To encode the representation of the floorplan boundary $\cI$, we follow ATISS and use an untrained ResNet-18~\cite{resnet} model to encode a top-down view of the layout boundary into a embedding vector.

\para{Training} During training, we create a ground truth sequence $S^\text{GT}$ with randomly permuted objects. We generate the condition $C$ as a copy of $S^\text{GT}$ and mask out a random percentage of the tokens by replacing them with the mask token $\mathcal{M}$. The boundary encoder $g^\mathcal{I}_\psi$, the condition encoder $g_\phi$ and the generative model $f_\theta$ are then trained jointly, with the task to generate the full sequence $S^\text{GT}$. For unmasked tokens in $C$, this is a copy task from $C$ to the output sequence $S$. For masked tokens, this is a scene completion task. We use the negative log-likelihood loss between the predicted probabilities $p(s_i)$ and ground truth values $s^\text{GT}_i$ for tokens corresponding to continuous parameters, and the cross-entropy loss for the object category $\tau$.
%using a ... \paul{TODO} loss.
The model is trained with teacher-forcing. 
% construct the sequence $S$ corresponding to the layout by arranging the object bounding boxes in a random order with a permutation $\pi$ and concatenating their bounding box attributes as individual tokens. \begin{equation}
%     s_1 = \texttt{SOS}, \;\;\; s_2 = \tau_{\pi_1}, \;\;\; s_3 = t_{\pi_1}, \;\;\; s_4 = e_{\pi_1}, \;\;\; s_5 = r_{\pi_1},  \;\;\; s_6 = \tau_{\pi_2}, \;\;\; \cdots \;\;\; s_k = \texttt{EOS}
% \end{equation}
% To construct the condition $C$, we drop the \texttt{SOS} and \texttt{EOS} tokens and randomly mask out a random ratio of the tokens in the remaining sequence. We prepend the boundary representation $\cI$ from the Boundary Encoder to the other embeddings.  The overall model is trained with teacher-forcing.

% Now we describe how the transformed-based generative model $f_\theta$ and the transformed encoder $g_\phi$ are implemented.
% %Now we describe how each of the parts in the objective Eq. \ref{eq:final_objective} are implemented.
% On a high level, we use a BART-like model for generation. We want the conditioning to be permutation-invariant, hence we remove absolute positional embeddings from the encoder. These are present in the decoder. BART is often used for machine translation, and in that setting usually receives the source language on the encoder, and target language on the decoder. We use BART for generation, and our encoder and decoder receive the same input, with some minor differences that we explain below. With our modifications the encoder represents a set (of conditions and masks), while the decoder samples a sequence. Thus, our task is a \textbf{Masked Set-to-Sequence prediction} task. 

% \para{Boundary Encoder} To encode the representation of the floorplan boundary $\cI$, we follow ATISS and use an untrained ResNet-18~\cite{resnet} model to encode a top-down view of the layout boundary into a embedding vector.

% \para{Set Encoder ($g_\phi$)} To encode the set representation $C^g$, we use a Transformer Encoder with full bidirectional attention. Without any form of positional encoding, a standard transformer is fully permutation invariant. However, we find that some prior knowledge is needed to yield good samples. We provide two such sources of injecting information: 1. \textbf{Object Index Tokens} ($\mathcal{O}^i$): We assign each object in the permuted set an index and 2. \textbf{Relative Position Tokens} ($\mathcal{R}^i$): To each attribute of an object, we assign a canonical position. Note that all these additional tokens are permutation-invariant. The embeddings for one attribute are generated by summing up all the corresponding embeddings. %

% \para{Sequence Decoder ($f_\theta$)} The sequence decoder implements autoregressive decoding and is a Transformer Decoder with a causal attention mask. It performs cross-attention into the activations of the final hidden layer of the Set Encoder. We reuse the \textit{unmasked} embeddings generated for encoder side, without embeddings for $\mathcal{R}^i$ and $\mathcal{O}^i$. Instead, we use full \textbf{Absolute Position Tokens} ($\mathcal{P}$) which is standard in Language Modelling. %The sequence is enclosed in \texttt{SOS} and \texttt{EOS} embeddings to denote the start and end of the sequence respectively.

% \para{Training} During training, we construct the sequence $S$ corresponding to the layout by arranging the object bounding boxes in a random order with a permutation $\pi$ and concatenating their bounding box attributes as individual tokens. \begin{equation}
%     s_1 = \texttt{SOS}, \;\;\; s_2 = \tau_{\pi_1}, \;\;\; s_3 = t_{\pi_1}, \;\;\; s_4 = e_{\pi_1}, \;\;\; s_5 = r_{\pi_1},  \;\;\; s_6 = \tau_{\pi_2}, \;\;\; \cdots \;\;\; s_k = \texttt{EOS}
% \end{equation}
% To construct the condition $C$, we drop the \texttt{SOS} and \texttt{EOS} tokens and randomly mask out a random ratio of the tokens in the remaining sequence. We prepend the boundary representation $\cI$ from the Boundary Encoder to the other embeddings.  The overall model is trained with teacher-forcing.

%Using Absolute Position Tokens on the Decoder and permutation-invariant Object Index Tokens and Relative Position Tokens on the Encoder makes the task a \textbf{Set-to-Sequence} task. Given a set of objects, we randomly assign an object index to each object. Then the Decoder should be able to use the relative position of each attribute to create a canonical sequence from that set. Refer for Fig. \ref{fig:architecture} for a visual representation.

% For a detailed description of the architecture and hyperparameters, please refer to the Appendix.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/sampling.pdf}\caption{\textbf{Sampling Strategy}. (\textbf{Left}): We start out with a sequence of all \mask tokens on the encoder, and the \texttt{SOS} token on the decoder. Conditions, if any, are specified by replacing the \mask with the desired value of the attribute in the sequence. Sampling is performed autoregressively. (\textbf{Right}): After a token has been sampled, both the encoder and decoder sequences are updated, and atuoregressive generation continues.}
    \label{fig:sampling}
\vspace{-0.5cm}
\end{figure*}

\para{Sampling}
% \subsection{Sampling}
%Sampling from Masked Language Models is an open problem~(\cite{wang-cho-2019-bert}). But our structured sequences allow for easier sampling.
%Specifically,
% We formulate sampling as a Neural Machine Translation (NMT) problem~(\cite{klein-etal-2017-opennmt}).
We generate a sequence auto-regressively, one token at a time, by sampling the probability distribution predicted by the generative model (as defined in Eq.~\ref{eq:final_objective}) in each step. We use the same model for both conditional and unconditional generation. For unconditional generation, we start with a condition $C$ where all tokens are mask token $\mathcal{M}$. To provide more complete information about the partially generated scene to the encoded condition tokens $C^g$, we update the condition $C$ after each generation step by replacing mask tokens with the generated tokens.
% as shown in Algorithm~\ref{alg:decoding}.
Empirically, we observed that this improves generation performance. An illustration of this approach is shown in Fig. \ref{fig:sampling}.
%To perform unconditional sampling, we start with encoding the floorplan boundary $\cI$, and set all condition tokens $C$ to $\mathcal{M}$. Then we sample autoregressively on the decoder. The only difference is that in NMT, the encoder pass is made only once and the decoder sequence is updated, but in our case every new sample replaces a \mask token in both the encoder and the decoder. In order to perform, conditional sampling, we simply replace \mask tokens in $C$ with the attributes we want.
The function \textsf{SAMPLE} samples from the probability distributions described in Eq.~\ref{eq:probab}.
% \vspace{-0.5cm}
%
% \begin{minipage}[h]{0.48\linewidth}
%     \small
%     \begin{algorithm}[H]
%       \caption{Standard Cond. Sampling}\label{alg:decoding}
%       \begin{algorithmic}[1]
%         \Require{$C = (c_i)_{i=1}^k$, $S = (\texttt{SOS}), s = \phi$}
%         \State {${C^g = g_\phi([\cI, C])}$} \Comment{Only performed once}
%         \While{$s \neq \texttt{EOS}$}% \Comment{Loop over semantic group}
%             \State {$s = \textsf{SAMPLE}(f_\theta(S_{<i}, C^g))$}
%             \State {$S\textsf{.append($s$)}$} \Comment{$C$ not updated}
%         \EndWhile
%         \State \textbf{return} $S$
%       \end{algorithmic}
%     \end{algorithm}
% \end{minipage}
% \begin{minipage}[h]{0.48\linewidth}
%     \small
%     \begin{algorithm}[H]
%       \caption{Our Sampling}\label{alg:decoding}
%       \begin{algorithmic}[1]
%         \Require{$\cI$, $C = (\mask)_{i=1}^k$, $S = (\texttt{SOS})$}
%         \For{$i \gets 1$ to $k$}% \Comment{Loop over semantic group}
%             \State {${\color{blue} C^g = g_\phi([\cI, C])}$}
%             \State {$s = \textsf{SAMPLE}(f_\theta(S_{<i}, C^g))$}
%             \State {${\color{blue} C[i] = s}, \; S\textsf{.append($s$)}$}
%         \EndFor
%         \State \textbf{return} $S$
%       \end{algorithmic}
%     \end{algorithm}
% \end{minipage}
%
% differently for different tokens (attributes) - softmax for the class label and a mixture of discretized logistics~(\cite{Salimans2017PixeCNN}) for the other attributes (see Eq. \ref{eq:probab}). 

Once a layout has been generated, we can populate the bounding boxes with objects from the dataset. For each bounding box, we pick the object of the given category $\tau$ that best matches the size of the bounding box. In the supplementary, we will present an ablation of the tokens $\mathcal{O}^i$, $\mathcal{R}^i$, and $\mathcal{P}$ that we add to the conditional encoder and generative model.
%in practice we pick the object that best matches the 

%After we have sampled a layout conditioned on a given floorplan boundary, we populate the layout by assigning the labeled bounding box with an object from the dataset that is closest to the generated bounding box in size. 





==> COFS_ Controllable Furniture Layout Synthesis/sections/related_work.tex <==
\section{Related Work}

\begin{table}[t]
\centering
\setlength\tabcolsep{2pt}
\resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}lcccccc@{}} 
    \toprule
    % \multicolumn{1}{l}{} & \multicolumn{4}{c}{CAS ($\downarrow$)}    & \multicolumn{4}{c}{KL-Divergence $\times 10^3$ ($\downarrow$)}       \\ \cmidrule(l){2-5} \cmidrule(l){6-9}
        & \makecell{Generative \\ Model}      & Sampling  & Representation &  Throughput &  \makecell{Likelihood\\ Estimation } & \makecell{Arbitrary \\ Conditioning} \\ \midrule
      FastSynth &        CNN+VAE               &        AR   & Set+Sequence &      Low          &      No       &              \xmark                                 \\
      SceneFormer &      Transformer              &      AR  & Sequence     &      Low          &     Yes        &            \xmark                                  \\
      ATISS  &           Transformer             &       AR   & Set &          High      &        Yes     &              \xmark                                 \\
      Ours &             Transformer               &      NAR/AR     &  Set &       High        &     Yes        &          \cmark                 \\
    
    \bottomrule
    \end{tabular}
}
\vspace{0.1cm}
\caption{\textbf{Comparison of our proposed model to other state-of-the art models}: Our model is the only model that can perform non-autoregressive sampling, has a set representation, is lightweight, can estimate the likelihood of an existing scene and also allows for arbitrary conditioning on any object parameter. }
\vspace{-0.8cm}
\end{table}


We discuss recent work that we draw inspiration from. In particular, we build on previous work in Indoor Scene Synthesis, Masked Language Models, and Set Transformers.

\para{Indoor Scene Synthesis} Before the rise of deep-learning methods, indoor scene synthesis methods relied on layout guidelines developed by skilled interior designers, and an optimzation strategy such that the adherence to those guidelines is maximized~\cite{makeithome:yu, example_furniture:fisher, scalable:weiss}. Such optimization is usually based on sampling methods like simulated annealing, MCMC, or rjMCMC. Deep learning based methods, e.g.~\cite{planit:wang, fastsynth:ritchie, wang2021sceneformer, Paschalidou2021NEURIPS} are substantially faster and can better capture the variability of the design space. The state-of-the-art methods among them are autoregressive in nature. All of these  operate on a top-down view of a partially generated scene. PlanIT and FastSynth then autoregressively generate the rest of the scene. FastSynth uses separate CNNs+MLPs to create probability distributions over location, size and orientation and categories. PlanIT on the other hand generates graphs where nodes are objects and edges are constraints on those objects. Then a scene is instantiated by solving a CSP on that graph.

Recent methods, SceneFormer~\cite{wang2021sceneformer} and ATISS~\cite{Paschalidou2021NEURIPS} use transformer based architectures to sidestep the problem of rendering a partial scene which makes PlanIT and FastSynth slow. This is because using a transformer allows the model to accumulate information from previously generated objects using the attention mechanism. SceneFormer flattens the scene into a structured sequence of the object attributes, where the objects are ordered lexicographically in terms of their position. It then trains a separate model for each of the attributes. ATISS breaks the requirement of using a specific order by training on all possible permutations of the object order and removing the position encoding. In addition, it uses a single transformer model for all attributes and relies on different decoding heads which makes it substantially faster than other models while also having significantly fewer parameters.

\para{Masked Language Models} Masked Language Models (MLMs) like BERT~\cite{devlin-etal-2019-bert}, ROBERTa~\cite{liu2019roberta}, and BART~\cite{lewis-etal-2020-bart} have been very successful in pre-training for language models. These models are pretrained on large amounts of unlabeled data in an unsupervised fashion, and are then fine-tuned on a much smaller labeled dataset. These fine-tuned models show impressive performance on their corresponding downstream tasks. However, the generative capability of these models has not been much explored except by Wang et al. in \cite{wang2019bert}, which uses a Gibbs-sampling approach to sample from a pre-trained BERT model. Follow up work in Mansimov et al.~\cite{mansimov2020a}, proposes more general sampling approaches. However, the sample quality is still inferior to autoregressive models like GPT-2~\cite{radford2019language} and GPT-3~\cite{brown2020language}.
More recently, MLMs have received renewed interest especially in the context of image-generation~\cite{issenhuth2021edibert, chang2022maskgit}. MaskGit~\cite{chang2022maskgit} shows that with a carefully designed masking schedule, high quality image samples can be generated from MLMs with parallel sampling which makes them much faster than autoregressive models. Edi-BERT~\cite{issenhuth2021edibert} shows that the BERT masking objective can be succesfully used with a VQGAN~\cite{taming} representation of an image to perform high quality image editing. Our model most closely resembles BART when used as a generative model.

\para{Set Transfomers} Zaheer et al.~\cite{deepsets} introduced a framework called DeepSets providing a mathematical foundation for networks operating on set-structured data. A key insight is that operations in the network need to be permutation invariant. Methods based on such a formulation were extremely successful, especially in the context of point-could processing~\cite{pointnet, ravanbakhsh2016deep}. Transformer models without any form of positional encoding are permutation invariant by design. Yet, almost all the groundbreaking works in transformers use some from of positional encoding, as in objection detection~\cite{detr}, language generation~\cite{radford2019language, brown2020language}, and image-generation~\cite{chang2022maskgit}. One of the early attempts to use a truly permutation invariant set transformer was in Set Transformer~\cite{lee2019set}, who methodically designed  principled operations that are permutation invariant but could only achieve respectable performance in toy-problems. However, recent work based on \cite{lee2019set} shows impressive performance in 3d-Object Detection~\cite{he2022voxset}, 3d Pose Estimation~\cite{ugrinovic2022permutation}, and SFM~\cite{moransfm}. 

==> COFS_ Controllable Furniture Layout Synthesis/sections/results.tex <==
\section{Results}

\begin{table}[b]
\centering
% \small
\caption{\textbf{Comparison on Unconditional Generation}: We provide floorplan boundaries from the Ground Truth as an input to the methods and compare the quality of generate scenes. We measure the CAS at a resolution of $256\times256$.We retrain the ATISS model and report the new numbers. The retrained model is called ATISS$^{*}$. The KL-Divergence follows from \cite{fastsynth:ritchie} and is the categorical KL-divergence between the distribution of classes in the GT and the layouts synthesised by our method.}
\setlength\tabcolsep{2pt}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\multicolumn{1}{l}{} & \multicolumn{4}{c}{CAS $\times 10^2$($\downarrow$)}    & \multicolumn{4}{c}{KL-Divergence $\times 10^3$ ($\downarrow$)}       \\ \cmidrule(l){2-5} \cmidrule(l){6-9}
                                    & \bed      & \liv & \din &  \lib                         & \bed & \liv & \din & \lib \\ \midrule
\multicolumn{1}{l}{FastSynth}       & 88.3        & 94.5  & 93.5  &  \multicolumn{1}{c|}{81.5}      & 6.4   & 17.6   & 51.8   & 43.1    \\
\multicolumn{1}{l}{SceneFormer}     & 94.5        & 97.2  & 94.1  &  \multicolumn{1}{c|}{88.0}      & 5.2     & 31.3   & 36.8   & 23.2    \\
\multicolumn{1}{l}{ATISS$^*$}       & 61.1       & \textbf{76.4}  & \textbf{69.1}  &  \multicolumn{1}{c|}{\textbf{61.77}}      & 8.6     & 14.1   & 15.6   & 10.1      \\%
%
% Our rows from here on
% \multicolumn{1}{l}{Ours+Cosine}     & -            &             &       & \multicolumn{1}{l|}{}     &                      &             &       &\\
\multicolumn{1}{l}{Ours}            & \textbf{61.0}            &    78.9         &    76.1   &  \multicolumn{1}{c|}{66.2}   &   \textbf{5.0}                   &   \textbf{8.1}          &    \textbf{9.3}   & \textbf{6.7} \\

\bottomrule
\end{tabular}
\vspace{0.1cm}
\end{table}


\begin{figure*}[t!]

    \centering
    \vspace{-1.5em}
    % \hfill
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
	    \small Boundary
    \end{subfigure}%
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
        \small GT
    \end{subfigure}%
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
        \small ATISS
    \end{subfigure}%
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
        \small Ours
    \end{subfigure}%
    % \hfill%
    \vskip\baselineskip%
    \vspace{-0.75em}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % \hfill
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
	    \includegraphics[width=\textwidth, trim=0 500 0 600, clip]{figures/unconstrained/LivingDiningRoom-6844_outline_orthopng.jpg}
    \end{subfigure}%
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
        % \begin{mdframed}[backgroundcolor=yellow!25, linewidth=0]
            \begin{overpic}[width=\textwidth,  trim=0 500 0 600, clip]{figures/unconstrained/LivingDiningRoom-6844_gt_orthopng.jpg}
        \end{overpic}
        % \end{mdframed}
    \end{subfigure}%
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
        \begin{overpic}[width=\textwidth,  trim=0 500 0 600, clip]{figures/unconstrained/LivingDiningRoom-6844_atiss_orthopng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
        \begin{overpic}[width=\textwidth, trim=0 500 0 600, clip]{figures/unconstrained/LivingDiningRoom-6844_orthopng.jpg}
        \end{overpic}
    \end{subfigure}%
    % \hfill%
    \vskip\baselineskip%
    \vspace{-0.75em}
    % \hfill
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
	    \includegraphics[width=\textwidth, trim=530 380 100 600, clip]{figures/unconstrained/LivingDiningRoom-20487_outline_orthopng.jpg}
    \end{subfigure}%
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
        \begin{overpic}[width=\textwidth,  trim=530 380 100 600, clip]{figures/unconstrained/LivingDiningRoom-20487_gt_orthopng.jpg}
        \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
        \begin{overpic}[width=\textwidth,  trim=530 380 100 600,
        clip]{figures/unconstrained/LivingDiningRoom-20487_atiss_orthopng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.22\linewidth}
        \begin{overpic}[width=\textwidth,  trim=530 380 100 600, clip]{figures/unconstrained/LivingDiningRoom-20487_orthopng.jpg}
        \end{overpic}
    \end{subfigure}%
    % \hfill%
    \vskip\baselineskip%
    \vspace{-0.75em}
    % \hfill
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
	    \includegraphics[width=\textwidth,  trim=550 600 600 550, clip]{figures/unconstrained/DiningRoom-10302_outline_orthopng..jpg}
    \end{subfigure}%
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
        \begin{overpic}[width=\textwidth,  trim=550 600 600 550, clip]{figures/unconstrained/dinner_orthopng.jpg}
        \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
        \begin{overpic}[width=\textwidth,  trim=550 600 600 550,
        clip]{figures/unconstrained/DiningRoom-10302_atiss_orthopng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.22\linewidth}
        \begin{overpic}[width=\textwidth,  trim=550 600 600 550, clip]{figures/unconstrained/DiningRoom-10302_orthopng.jpg}
        \end{overpic}
    \end{subfigure}%
    % \hfill%
    \vskip\baselineskip%
    \vspace{-0.75em}
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
	    \includegraphics[width=\textwidth,  trim=530 380 300 600, clip]{figures/unconstrained/LivingDiningRoom-2648_outline_orthopng.jpg}
    \end{subfigure}%
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
        \begin{overpic}[width=\textwidth,  trim=530 380 300 600, clip]{figures/unconstrained/LivingDiningRoom-2648_gt_orthopng.jpg}
        \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
        \begin{overpic}[width=\textwidth,  trim=530 380 300 600,
        clip]{figures/unconstrained/LivingDiningRoom-2648_atiss_orthopng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.22\linewidth}
        \begin{overpic}[width=\textwidth,  trim=530 380 300 600, clip]{figures/unconstrained/LivingDiningRoom-2648_orthopng.jpg}
        \end{overpic}
    \end{subfigure}%
    
    \caption{\textbf{Scene generation from scratch:} We compare generated scenes from GT, ATISS, and our model. Both ATISS and our model are conditioned on the floorplan boundary (first column). In contrast to ATISS, we can see that our model consistently creates plausible layouts within the floorplan boundary while avoiding unnatural object intersections. These are results on the challenging \liv (rows 1,3) and \din (row 2,4) categories. Additional results can be found in the supplementary. (Best viewed zoomed in, on a computer display)}
    \label{fig:qualitative_gen_from_scratch}
\vspace{-0.75em}
\end{figure*}

\subsection{Experimental Setup}

\para{Datasets} We train and evaluate our model on the 3D-FRONT dataset. It consists of of about $10k$ indoor scenes created by professional designers. We follow ATISS preprocessing which removes a few problematic scenes that have intersections between objects, or mislabeled objects, or scenes that have extremely large or small dimensions. For further details on the preprocessing, we refer the reader to ATISS~\cite{Paschalidou2021NEURIPS}. We train on the following classes of rooms - \bed, \lib, \din, \liv. We closely follow the preprocessing step of ATISS, yielding approximately $6k$, $0.6k$, $3k$ and $2.6k$ scenes for \bed, \lib, \din, \liv respectively. These classes have substantially different numbers of layouts and numbers of objects per layout. %Consequently, we train models of different sizes for each of the classes. %For detailed architectural details, please refer to the Appendix.

\para{Hyperparameters} We implement our models in PyTorch~\cite{pytorch} 1.7.0. We use standard transformer blocks for the encoder and decoder except that the ReLU activation is replaced with GeLU~\cite{gelu}. We use 4 encoder layers and 4 decoder layers, with a hidden dimension of 256 and 4 attention heads yielding a query vector of dimension 64. We use a batch size of 128 sequences and train on a single nVIDIA A100 GPU with the AdamW~\cite{loshchilov2018decoupled_adamw} optimizer which we found to be more stable than Adam~\cite{adam_kingma}. We use weight decay of 0.001 and clip the gradient norm to be a maximium of 30. We found that the networks begins to overfit very early, especially for classes other than \bed, because of the scarcity of data. Thus, for training networks on other classes, we pre-train on the \bed class, and then reuse those weights as initialization. We do not use any form of learning rate scheduling as our experiments did not suggest significant performance gains. We train for 1000 epochs and use early stopping.

\para{Baselines} Our main comparison is with respect to ATISS, as they are the only other method that considers the layout generation problem in a permutation invariant set-generation setting. We show that our model is competitive with ATISS and outperforms it on certain metrics. Moreover, we subsume all functionality of ATISS, including partial scene completion and outlier detection. Unlike ATISS, our model allows for fine-grained conditioning on arbitrary object parameters. 

%As an added advantage, our model sidesteps the autoregressive ordering for the generation of object parameters and allows for conditioning on any arbitrary object parameter.
ATISS does not provide pretrained models, hence we train their models using the official code \footnote{ \href{https://github.com/nv-tlabs/atiss}{https://github.com/nv-tlabs/atiss}, commit \texttt{0cce45b
}} and match their training settings as closely as possible. Further, we compare to previous state-of-the art methods, FastSynth~\cite{fastsynth:ritchie} and SceneFormer~\cite{wang2021sceneformer} quantitatively. % We additionally also compare against cite niessner cite ritchie and show that our model outperforms those baselines by a significant margin.

\para{Metrics} Our metrics mostly derive from \cite{fastsynth:ritchie, Paschalidou2021NEURIPS}. Following, \cite{fastsynth:ritchie}, we report the KL-divergence between the distribution of the classes of generated objects and the distribution of classes of the objects in the test set. We further report the Classification Accuracy Score (CAS)~\cite{Paschalidou2021NEURIPS}. We render the the populated layout from a top-down view using an orthographic camera at a resolution of $256 \times 256$. We report the FID computed between these rendered top down images of sampled layouts and the renders of the ground truth layouts.

% While cite despoina report the FID, we do not report the FID as we found it to be very unreliable and sensitive to the rendering style. . In order to test this, we computed the FID between the validation and test sets of the \bed class and found out the FID to be $80.4$ (TODO confirm) which is greater than reported by cite despoina. 

% FID is known to be meaningless especially for small datasets and none of our test sets had greater than $500$ samples

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}


% \begin{table}[t!]
% \centering
% \small
% \setlength\tabcolsep{2pt}
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule
% \multicolumn{1}{l}{} & \multicolumn{4}{c}{CAS $\times 10^2$($\downarrow$)}    & \multicolumn{4}{c}{KL-Divergence $\times 10^3$ ($\downarrow$)}       \\ \cmidrule(l){2-5} \cmidrule(l){6-9}
%                                     & \bed      & \liv & \din &  \lib                         & \bed & \liv & \din & \lib \\ \midrule
% \multicolumn{1}{l}{ATISS$^{*}$}           & 38.39        & 33.14  & 29.23  &  \multicolumn{1}{l|}{35.60}      & 8.5     & 3.4    & 6.1    & 9.8     \\%
% %
% % Our rows from here on
% \multicolumn{1}{l}{Ours+Cosine}     & -            &             &       & \multicolumn{1}{l|}{}     &                      &             &       &\\
% \multicolumn{1}{l}{Ours}            & -            &             &       &  \multicolumn{1}{l|}{}   &                      &             &       & \\

% \bottomrule
% \end{tabular}
% \vspace{0.1cm}
% \caption{\textbf{Comparison on Conditional Generation}: We provide partial scenes from the Ground Truth as an input to the methods and compare the quality of generate scenes. We measure the CAS at a resolution of $256\times256$. The KL-Divergence is measured between the distribution of object categories in the Ground Truth vs. our generated samples. ATISS does not report the these metrics for conditional generation, so we retrain their model and report these numbers. The retrained model is called ATISS$^{*}$. The KL-Divergence follows from the \cite{fastsynth:ritchie} and is the categorical KL-divergence between the distribution of classes in the GT and the layouts synthesised by our method.}
% \end{table}





    
\subsection{Applications}
In this section, we discuss the application of our model on multiple interactive tasks. We show that our formulation a) can perform the same tasks as existing models and b) additionally enables fine-grained conditioning on arbitrary sequence subsets, like individual object parameters. % To the best of our knowledge we propose the first layout generation method to do so.
% which no existing model in the literature can, to the best of our knowledge.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\para{Scene Completion} In order to perform scene completion, we prepend both $S$ and $C$ with the tokens of the objects that already exist in the scene. Examples are shown in Figure~\ref{fig:partial_scene_completion}. We can see that our method successfully generates plausible room layouts that respect the condition shown in the top row.

\begin{figure*}[t!]
    \centering
    \vspace{-1.5em}
    % \hfill
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
	    \begin{overpic}[width=\linewidth,  trim=640 600 600 900, clip]{figures/completions/partial_1_westpng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
        \begin{overpic}[width=\textwidth,  trim=600 600 600 760, clip]{figures/completions/partial_2_eastpng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
        \vspace{-3mm}
        \begin{overpic}[width=\textwidth,  trim=600 600 600 700, clip]{figures/completions/partial_3_eastpng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
        \begin{overpic}[width=\textwidth,  trim=550 700 500 500, clip]{figures/completions/partial_4_northpng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
    \begin{overpic}[width=\textwidth,  trim=500 600 500 550 , clip]{figures/completions/partial_5_northpng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
            \begin{overpic}[width=\textwidth,  trim=600 700 600 550, clip]{figures/completions/partial_6_northpng.jpg}
        \end{overpic}
    \end{subfigure}%
    \vskip\baselineskip%
    \vspace{-1.75em}
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
	    \begin{overpic}[width=\linewidth,  trim=640 600 600 900, clip]{figures/completions/completed_1_westpng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
        \begin{overpic}[width=\textwidth,  trim=600 600 600 760, clip]{figures/completions/completed_2_eastpng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
        \begin{overpic}[width=\textwidth,  trim=600 600 600 700, clip]{figures/completions/completed_3_eastpng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
        \begin{overpic}[width=\textwidth,  trim=550 700 500 500, clip]{figures/completions/complete_4_northpng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
    \begin{overpic}[width=\textwidth,  trim=500 600 500 550, clip]{figures/completions/complete_5_northpng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
            \begin{overpic}[width=\textwidth,  trim=600 700 600 550, clip]{figures/completions/complete_6_northpng.jpg}
        \end{overpic}
    \end{subfigure}%
    \caption{\textbf{Partial Scene Completion:} We show qualitative visualizations for the scene completion task. The generated layouts all respect the condition they were generated with (top row) and are all plausible room layouts.}
    \label{fig:partial_scene_completion}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\para{Outlier Detection} To estimate the likelihood of each token, we follow \cite{salazar-etal-2020-masked} and replace the token at $i$th position with \mask. This can be performed in parallel by creating a batch in which only one element is replaced with \mask. This is shown in Fig. \ref{fig:architecture}. The likelihood of one bounding box then is the product of likelihoods of all element of the bounding box. Objects with low likelihood can then be resampled. Based on user constraints, only one parameter may be changed as we allow for arbitrary conditioning as explained in the next section.

\begin{figure*}[b]
    \centering
    \vspace{-1.5em}
    % \hfill
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
	    \begin{overpic}[width=\linewidth,  trim=500 500 500 500, clip]{figures/outlier/bad_last_sepng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
        \begin{overpic}[width=\textwidth,  trim=500 500 500 500, clip]{figures/outlier/bad1_sepng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
        \vspace{-3mm}
        \begin{overpic}[width=\textwidth,  trim=100 300 400 700, clip]{figures/outlier/bad2_eastpng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
        \begin{overpic}[width=\textwidth,  trim=400 300 400 650, clip]{figures/outlier/bad3_sepng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
    \begin{overpic}[width=\textwidth,  trim=100 200 200 500, clip]{figures/outlier/bad4_nepng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
            \begin{overpic}[width=\textwidth,  trim=100 400 400 550, clip]{figures/outlier/bad5_nwpng.jpg}
        \end{overpic}
    \end{subfigure}%
    \vskip\baselineskip%
    \vspace{-1.75em}
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
	    \begin{overpic}[width=\linewidth,  trim=500 500 500 500, clip]{figures/outlier/good_last_sepng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
        \begin{overpic}[width=\textwidth,  trim=500 500 500 500, clip]{figures/outlier/good1_sepng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
        \begin{overpic}[width=\textwidth,  trim=100 300 400 700, clip]{figures/outlier/good2_eastpng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
        \begin{overpic}[width=\textwidth,  trim=400 300 400 650, clip]{figures/outlier/good3_sepng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
    \begin{overpic}[width=\textwidth,  trim=100 200 200 500, clip]{figures/outlier/good4_nepng.jpg}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.16\linewidth}
        \centering
            \begin{overpic}[width=\textwidth,  trim=100 400 400 550, clip]{figures/outlier/good5_nwpng.jpg}
        \end{overpic}
    \end{subfigure}%
    
    \caption{\textbf{Outlier detection:} Our model can utilize bidirectional attention to reason about unlikely arrangements of furniture. We can then sample new attributes that create a more likely layout. \textbf{Top row:} An object is perturbed to create an outlier (highlighted in blue). \textbf{Bottom row:} The object can be identified by its low likelihood, and new attributes sampled which place it more naturally. Please zoom in for best viewing.}
    \label{fig:outlier_detection}
\vspace{-0.75em}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\para{Arbitrary Conditioning}  
To condition on an arbitrary sub-set of object attributes, we can construct a condition $C$ that is filled with \mask tokens, i.e. a fully unconstrained setting, and then only replace the tokens in $C$ corresponding to the attributes we want to constrain with constraint values. The non-mask tokens do not need to be contiguous in $C$. Any subset of $C$, for example only object class attributes or only object locations, can be used as unmasked condition. Given such a constraint $C$, the generator proceeds as described in Section~\ref{sec:implementation} and fills in all mask tokens with generated values. The encoder allows each generation step to have full knowledge of the condition $C$. See Fig.~\ref{fig:arbitrary_cond} for examples.
%
%We sample autoregressively - first class, then translation, size and angle. Yet, as described in Section 3, our model has bidirectional attention on all encoder tokens. Thus, at inference time, we can replace any token with a \mask token and allow the network to estimate the likelihood of the \mask token under the current parameters. This can be used for arbitrary conditioning in the following manner, say we want to add an object to a scene - we append a sequence of \mask tokens to the existing sequence. Then in order to specify the class, location, size or angle of the desired object we just replace the corresponding \mask token and allow the network to predict the distributions of the remaining parameters. We show a few examples in Fig. \cite{fig:arbitrary_cond}. This allows the network to \textit{look-ahead} and \textit{see} what parameters to generate in the future, enabling it to change the current probabilities accordingly.
To the best of our knowledge, ours is the first model that allows for this form of conditioning without imposing an order on the generation of parameters.

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
	    \includegraphics[width=\textwidth, trim=450 500 500 450, clip]{figures/conditioning/condition/cabinet_northpng.png}
    \end{subfigure}%
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
            \begin{overpic}[width=\textwidth,  trim=450 500 500 450, clip]{figures/conditioning/cabinets_northpng.png}
        \end{overpic}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
        \begin{overpic}[width=\textwidth,  trim=450 500 500 450, clip]{figures/conditioning/condition/chair_northpng.png}
	    \end{overpic}
    \end{subfigure}%
    \begin{subfigure}[b]{0.22\linewidth}
        \centering
        \begin{overpic}[width=\textwidth, trim=450 500 500 450, clip]{figures/conditioning/chairs_northpng.png}
        \end{overpic}
    \end{subfigure}%
    \vskip\baselineskip%
    \vspace{-0.75em}
    \caption{\textbf{Arbitrary conditioning:} We constrain the location of the next object to be sampled. The location is highlighted in pink. We sample location after the class. In a normal autoregressive model, we would not be able to constrain on the location. The bidirectional attention in the encoder allows the network to generate \textit{current} tokens based on \textit{future} tokens. In this example, the network automatically infers the proper class and size and even matches the style of the chairs in the example on the left.} 
    \label{fig:arbitrary_cond}
    
\end{figure*}




==> COFS_ Controllable Furniture Layout Synthesis/symbols.tex <==
\newcommand{\ba}{\mathbf{a}}\newcommand{\bA}{\mathbf{A}}
\newcommand{\bb}{\mathbf{b}}\newcommand{\bB}{\mathbf{B}}
\newcommand{\bc}{\mathbf{c}}\newcommand{\bC}{\mathbf{C}}
\newcommand{\bd}{\mathbf{d}}\newcommand{\bD}{\mathbf{D}}
\newcommand{\be}{\mathbf{e}}\newcommand{\bE}{\mathbf{E}}
\newcommand{\bff}{\mathbf{f}}\newcommand{\bF}{\mathbf{F}}
\newcommand{\bg}{\mathbf{g}}\newcommand{\bG}{\mathbf{G}}
\newcommand{\bh}{\mathbf{h}}\newcommand{\bH}{\mathbf{H}}
\newcommand{\bi}{\mathbf{i}}\newcommand{\bI}{\mathbf{I}}
\newcommand{\bj}{\mathbf{j}}\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bk}{\mathbf{k}}\newcommand{\bK}{\mathbf{K}}
\newcommand{\bl}{\mathbf{l}}\newcommand{\bL}{\mathbf{L}}
\newcommand{\bm}{\mathbf{m}}\newcommand{\bM}{\mathbf{M}}
\newcommand{\bn}{\mathbf{n}}\newcommand{\bN}{\mathbf{N}}
\newcommand{\bo}{\mathbf{o}}\newcommand{\bO}{\mathbf{O}}
\newcommand{\bp}{\mathbf{p}}\newcommand{\bP}{\mathbf{P}}
\newcommand{\bq}{\mathbf{q}}\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\br}{\mathbf{r}}\newcommand{\bR}{\mathbf{R}}
\newcommand{\bs}{\mathbf{s}}\newcommand{\bS}{\mathbf{S}}
\newcommand{\bt}{\mathbf{t}}\newcommand{\bT}{\mathbf{T}}
\newcommand{\bu}{\mathbf{u}}\newcommand{\bU}{\mathbf{U}}
\newcommand{\bv}{\mathbf{v}}\newcommand{\bV}{\mathbf{V}}
\newcommand{\bw}{\mathbf{w}}\newcommand{\bW}{\mathbf{W}}
\newcommand{\bx}{\mathbf{x}}\newcommand{\bX}{\mathbf{X}}
\newcommand{\by}{\mathbf{y}}\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bz}{\mathbf{z}}\newcommand{\bZ}{\mathbf{Z}}

\newcommand{\balpha}{\boldsymbol{\alpha}}\newcommand{\bAlpha}{\boldsymbol{\Alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}\newcommand{\bBeta}{\boldsymbol{\Beta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\bdelta}{\boldsymbol{\delta}}\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}\newcommand{\bEpsilon}{\boldsymbol{\Epsilon}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}\newcommand{\bZeta}{\boldsymbol{\Zeta}}
\newcommand{\beeta}{\boldsymbol{\eta}}\newcommand{\bEta}{\boldsymbol{\Eta}} \newcommand{\btheta}{\boldsymbol{\theta}}\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\biota}{\boldsymbol{\iota}}\newcommand{\bIota}{\boldsymbol{\Iota}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}\newcommand{\bKappa}{\boldsymbol{\Kappa}}
\newcommand{\blambda}{\boldsymbol{\lambda}}\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}\newcommand{\bMu}{\boldsymbol{\Mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}\newcommand{\bNu}{\boldsymbol{\Nu}}
\newcommand{\bxi}{\boldsymbol{\xi}}\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\bomikron}{\boldsymbol{\omikron}}\newcommand{\bOmikron}{\boldsymbol{\Omikron}}
\newcommand{\bpi}{\boldsymbol{\pi}}\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\brho}{\boldsymbol{\rho}}\newcommand{\bRho}{\boldsymbol{\Rho}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\btau}{\boldsymbol{\tau}}\newcommand{\bTau}{\boldsymbol{\Tau}}
\newcommand{\bypsilon}{\boldsymbol{\ypsilon}}\newcommand{\bYpsilon}{\boldsymbol{\Ypsilon}}
\newcommand{\bphi}{\boldsymbol{\phi}}\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bchi}{\boldsymbol{\chi}}\newcommand{\bChi}{\boldsymbol{\Chi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bomega}{\boldsymbol{\omega}}\newcommand{\bOmega}{\boldsymbol{\Omega}}

\newcommand{\nA}{\mathbb{A}}
\newcommand{\nB}{\mathbb{B}}
\newcommand{\nC}{\mathbb{C}}
\newcommand{\nD}{\mathbb{D}}
\newcommand{\nE}{\mathbb{E}}
\newcommand{\nF}{\mathbb{F}}
\newcommand{\nG}{\mathbb{G}}
\newcommand{\nH}{\mathbb{H}}
\newcommand{\nI}{\mathbb{I}}
\newcommand{\nJ}{\mathbb{J}}
\newcommand{\nK}{\mathbb{K}}
\newcommand{\nL}{\mathbb{L}}
\newcommand{\nM}{\mathbb{M}}
\newcommand{\nN}{\mathbb{N}}
\newcommand{\nO}{\mathbb{O}}
\newcommand{\nP}{\mathbb{P}}
\newcommand{\nQ}{\mathbb{Q}}
\newcommand{\nR}{\mathbb{R}}
\newcommand{\nS}{\mathbb{S}}
\newcommand{\nT}{\mathbb{T}}
\newcommand{\nU}{\mathbb{U}}
\newcommand{\nV}{\mathbb{V}}
\newcommand{\nW}{\mathbb{W}}
\newcommand{\nX}{\mathbb{X}}
\newcommand{\nY}{\mathbb{Y}}
\newcommand{\nZ}{\mathbb{Z}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\co}{\mathcal{o}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
